Instance-Optimality for Private KL Distribution Estimation

We study the fundamental problem of estimating an unknown discrete distribution $p$ over $d$ symbols, given $n$ i.i.d. samples from the distribution. We are interested in minimizing the KL divergence between the true distribution and the algorithm's estimate. We first construct minimax optimal private estimators. Minimax optimality however fails to shed light on an algorithm's performance on individual (non-worst-case) instances $p$ and simple minimax-optimal DP estimators can have poor empirical performance on real distributions. We then study this problem from an instance-optimality viewpoint, where the algorithm's error on $p$ is compared to the minimum achievable estimation error over a small local neighborhood of $p$. Under natural notions of local neighborhood, we propose algorithms that achieve instance-optimality up to constant factors, with and without a differential privacy constraint. Our upper bounds rely on (private) variants of the Good-Turing estimator. Our lower bounds use additive local neighborhoods that more precisely captures the hardness of distribution estimation in KL divergence, compared to ones considered in prior works.

==> packages_and_commands.tex <==
%\usepackage{times}
% \usepackage[numbers,compress]{natbib}
% \usepackage{authblk}        % authors
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[]{hyperref}
\usepackage{url}



% \usepackage{algorithm}  % for algorithms
% % \usepackage{algorithmic}
% \usepackage[noend]{algpseudocode}  % for algorithms
\RequirePackage{algorithm}
\RequirePackage{algorithmic}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ALGORITHMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TABLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{multirow}
\usepackage{booktabs}





% % Recommended, but optional, packages for figures and better typesetting:
\usepackage{xcolor}
\usepackage{adjustbox}
\usepackage{tabularx}
\usepackage{subcaption}

% % Recommended, but optional, packages for figures and better typesetting:
% \usepackage{microtype}
\usepackage{graphicx}
% \usepackage{subfigure}
% \usepackage{booktabs} % for professional tables

% % hyperref makes hyperlinks in the resulting PDF.
% \usepackage{hyperref}


% % Attempt to make hyperref and algorithmic work together better:
% \newcommand{\theHalgorithm}{\arabic{algorithm}}


% For theorems and symbols 
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{bm}
\usepackage{enumitem}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage[textsize=tiny]{todonotes}

\pdfpagewidth 8.5in
\pdfpageheight 11in

\newcommand{\paragraphbe}[1]{\vspace{0.08in} \noindent{\bf \em #1}. }


% for tikz plots
%Set to 1 to compile Figures
\def\compileFigures{0}
\newcommand{\filename}{main}
\newcounter{figureNumber}


\usepackage{tikz}
\if\compileFigures1
\usetikzlibrary{external}
\tikzexternalize[prefix=fig/] % activate!
\fi

% figure template
% \begin{figure}
% 	\centering
% 	\if\compileFigures1
% 	\input{figure_scripts/fig_<meaningful_filename>}
% 	\else
% 	\includegraphics[]{fig/\filename-figure\thefigureNumber.pdf}
% 	\stepcounter{figureNumber}
% 	\fi
% 	\caption{<meaningful_caption>}
% 	\label{fig:<meaningful_label>}
% \end{figure}



\usepackage{tikz-cd}
\usetikzlibrary{calc}
\usepackage{pgfplots}
\usetikzlibrary{math}
\usepgfplotslibrary{groupplots}
\pgfplotsset{compat=1.3}
\usepackage{csvsimple}

% For Repeating Theorems Lemmas etc. in Appendix
\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{\bfseries #2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother

\newreptheorem{theorem}{Theorem}
\newreptheorem{lemma}{Lemma}
\newreptheorem{proposition}{Proposition}
\newreptheorem{corollary}{Corollary}

\usepackage{bm}



\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bx}{\mathbf x}
\newcommand{\by}{\mathbf y}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\inp}[2]{\ensuremath{\langle{#1},{#2}\rangle}}
\newcommand{\cL}{\mathcal L}
\DeclareMathOperator{\R}{\mathbb{R}}
\newcommand{\cA}{\mathcal A}
\newcommand{\eg}{\emph{e.g.}\;}
\newcommand{\ie}{\emph{i.e.}\;}


\usepackage{wrapfig}

\newdimen\figrasterwd
\figrasterwd\textwidth


\newcommand{\jy}[1]{\textcolor{red}{#1}}



\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
    \node[shape=circle,draw,inner sep=1.5pt] (char) {#1};}}

\usepackage{caption}
\captionsetup{font=small}
